Limits to Rest-Frame Ultraviolet Emission From Far-Infrared-Luminous z~6 Quasar Hosts

We report on a Hubble Space Telescope search for rest-frame ultraviolet emission from the host galaxies of five far-infrared-luminous $z\simeq{}6$ quasars and the $z=5.85$ hot-dust free quasar SDSS J0005-0006. We perform 2D surface brightness modeling for each quasar using a Markov-Chain Monte-Carlo estimator, to simultaneously fit and subtract the quasar point source in order to constrain the underlying host galaxy emission. We measure upper limits for the quasar host galaxies of $m_J>22.7$ mag and $m_H>22.4$ mag, corresponding to stellar masses of $M_\ast<2\times10^{11}M_\odot$. These stellar mass limits are consistent with the local $M_{\textrm{BH}}$-$M_\ast$ relation. Our flux limits are consistent with those predicted for the UV stellar populations of $z\simeq6$ host galaxies, but likely in the presence of significant dust ($\langle A_{\mathrm{UV}}\rangle\simeq 2.6$ mag). We also detect a total of up to 9 potential $z\simeq6$ quasar companion galaxies surrounding five of the six quasars, separated from the quasars by 1.4''-3.2'', or 8.4-19.4 kpc, which may be interacting with the quasar hosts. These nearby companion galaxies have UV absolute magnitudes of -22.1 to -19.9 mag, and UV spectral slopes $\beta$ of -2.0 to -0.2, consistent with luminous star-forming galaxies at $z\simeq6$. These results suggest that the quasars are in dense environments typical of luminous $z\simeq6$ galaxies. However, we cannot rule out the possibility that some of these companions are foreground interlopers. Infrared observations with the James Webb Space Telescope will be needed to detect the $z\simeq6$ quasar host galaxies and better constrain their stellar mass and dust content.

==> tables/tab_sfr.tex <==
\begin{deluxetable*}{llll}
\tablecolumns{4}
\tablewidth{0pt}
\tablecaption{Quasars Observed with HST}
\tablehead{
\colhead{Quasar Name} &
\colhead{Redshift} &
\colhead{$M_{1450}$ \n(mag)} &
\colhead{$L_{FIR}$ \n$(10^{12}~\LSun{})$}
}
\startdata
CFHQS J003311.40--012524.9 & 6.13   & $-25.14$ & $2.6\pm{}0.8$ \\
SDSS J012958.51--003539.7  & 5.7787 & $-23.89$ & $5.2\pm{}0.9$ \\
ULAS J020332.39+001229.3  & 5.72   & $-26.26$ & $4.4\pm{}1.1$ \\
NDWFS J142516.30+325409.0 & 5.8918 & $-26.47$ & $5.4\pm{}1.2$ \\
SDSS J205406.42--000514.8  & 6.0391 & $-26.21$ & $5.5\pm{}1.2$ \\
SDSS J000552.34--000655.8  & 5.85   & $-25.73$ & \nodata{}     \\
\enddata
\tablecomments{Quasar names include the full sexagesimal coordinates. Redshifts
and absolute magnitudes use the same references as Table 7 in
\citet{banados_pan-starrs1_2016}. FIR luminosities are from \citet{
wang_molecular_2010, wang_far-infrared_2011}.}
\label{tab_targets}
\end{deluxetable*}

